Removing Radio Frequency Interference from Auroral Kilometric Radiation with Stacked Autoencoders

Radio frequency data in astronomy enable scientists to analyze astrophysical phenomena. However, these data can be corrupted by radio frequency interference (RFI) that limits the observation of underlying natural processes. In this study, we extend recent developments in deep learning algorithms to astronomy data. We remove RFI from time-frequency spectrograms containing auroral kilometric radiation (AKR), a coherent radio emission originating from the Earth's auroral zones that is used to study astrophysical plasmas. We propose a Denoising Autoencoder for Auroral Radio Emissions (DAARE) trained with synthetic spectrograms to denoise AKR signals collected at the South Pole Station. DAARE achieves 42.2 peak signal-to-noise ratio (PSNR) and 0.981 structural similarity (SSIM) on synthesized AKR observations, improving PSNR by 3.9 and SSIM by 0.064 compared to state-of-the-art filtering and denoising networks. Qualitative comparisons demonstrate DAARE's capability to effectively remove RFI from real AKR observations, despite being trained completely on a dataset of simulated AKR. The framework for simulating AKR, training DAARE, and employing DAARE can be accessed at github.com/Cylumn/daare.

==> review/aurora.tex <==
\section{Aurora Lit Review}
\subsection{Auroral Kilometric Radiation}
\subsubsection{What are AKR}
\cite{labelle2002auroral} (Abstract) auroral electrons emit radio emissions with differing characteristics. Scientists have labeled them to be of four categories: AKR, Auroral Hiss, Auroral Roar, and high frequency emissions.

(Introduction) There's a lot of energy in the auroral ionosphere. This energy comes off as radiation. The mechanism believed to produce AKR is the "cyclotron maser mechanism". Non-AKR AR is much less powerful (< 0.1\% the energy of AKR).

\cite{labelle2011ground} (Abstract) AKR is emitted as up to 1\% of the Earth's auroral electron energy, produced through the electron cyclotron maser mechanism. First thought to not be capable of penetrating near the earth, occasional reports in the past few decades have detected AKR-like signals at low altitudes. This work compares AKR emissions detected on Geotail and from the South Pole.

(2) First identification: (Gurnett 1974) and first detection (Benedictov et al. 1966) and (Dunckel et al. 1970). It is an X-mode radiation with a minority O-mode component and emits in a conical radiation pattern. The total radiated power goes up to $10^9$ Watts. This is similar to powerful decametric radio emissions from Jupiter. Leaked AKR: (Oya et al. 1985). There are many different proposed mechanisms for why leaked AKR exists.

About the real data: (3) ``Dartmouth College operates several radio receivers at South Pole Station. There is a spectral analyzer covering 30-5000 kHz with a 10-kHz frequency resolution and 2-second time resolution. The sensor is a 10-meters squared loop antenna with an active preamp and is located about 1 km from the station. The receiver sensitivity is 5 $nV/mHz^{1/2}$, although station-generated radio interference often exceeds that level."

\subsubsection{Importance}

\cite{labelle2002auroral} (Introduction) EM waves enable sensing ionospheric plasma processes (by constraining ionospheric parameters such as electron density or gradient scale length). Studying Earth's auroras is a local way to investigate remote astrophysical plasmas where direct measurements are impossible and radiation is the only information source.

\cite{labelle2011ground} Other planets produce similar AKR-like emissions. 

\cite{erickson2018aero} (Abstract) Earth's aurora is of interest to improve our understanding of space physics. Studying auroral radio emissions in the LF and HF frequency range allow radio remote sensing and investigation of nonlinear wave processes and wave-particle interactions operating in heliospheric, planetary, and astrophysical plasmas. 

\subsection{Observation limitations}

\cite{labelle2002auroral} A subset of lower hybrid resonance (LHR) waves may represent payload generated noise rather than natural auroral hiss.

\cite{labelle2011ground} (3) "Antarctica is the best location for measuring natural radio waves at 30-1700 kHz due to the absence of local AM broadcast stations."

(5) Geotail detects weak interference lines and a phenomenon called kilometric continuum (Hashimoto et al. 1999) that consists of horizontally-structured emissions. The striped appearance of background noise and AKR is a result of a beat between the satellite spin and the swept frequency analyzer (SFA) sweep.

(Ganesh Rajagopalan's REU Talk): Other signals these instruments may detect: (1) cell phone towers, (2) local FM stations, (3) nearby TV stations, (4) DirecTV geo-stationary satellite, (5) NASA Spacecraft in the outer solar system

\subsection{AKR Structure}

\cite{labelle2002auroral} Auroral hiss often exhibits frequency and time fine structure, such as banding near harmonics of the ion gyrofrequency, wave localization, or dispersed bursts.

79\% of saucer emissions occur on field lines coincident with broadband electrostatic noise most likely caused by electron phase space holes.

\cite{labelle2011ground} The structure of AKR was important to establish ground-level detection of AKR.

\cite{erickson2018aero} Fine-scale AKR structure is an effective tool for remotely sensing the extent and dynamics of the auroral acceleration region (5-8).

(AERO SCIENCE HANDBOOK): ``Ground-level AKR is highly structured with variations over timescales of 100 ms. Escaping AKR is much finer around timescales of 10 Hz. 

==> review/denoising.tex <==
\section{Denoising Lit Review}
\subsection{Losses}
\cite{ma2020enhanced} : MSE
\\
\cite{zhao2018convolutional} : MSE
\\
\cite{huang2018micro} : DE + L1
\\
\cite{rethage2018wavenet} : L1
\\
\cite{zhang2016fast} : Weighted Euclidean
\\
\cite{li2019separating} : MSE
\\
\cite{zhang2018ffdnet} : MSE

\begin{table}[H]
    \renewcommand{\arraystretch}{1.3}
    \centering
    \caption{Losses used in similar papers.}
    \label{tab:lossdict}
    \begin{tabular}{p{0.2\linewidth}|p{0.5\linewidth}|p{0.15\linewidth}}
        \textbf{Acronym}&\textbf{Method}&\textbf{\# Uses}\\
        \toprule
        \bottomrule
        L1 & L1 Error & 1 (2)\\
        MSE & Mean Squared (Euclidean) Error & 4 (5)\\
        Weighted Euclidean & Custom Loss: Weighted Map * MSE Loss & 1\\
        DE & Discriminative (GAN) Error & 0 (1)\\
        \toprule
    \end{tabular}
\end{table}

\subsection{Baselines}
\cite{ma2020enhanced} : LRTA, BM4D, LRTV, LRMR, NMoG, and HSID-CNN
\\
\cite{zhao2018convolutional} : MS, DNN-SYMM, DNN-CAUSAL, RNN-NG
\\
\cite{huang2018micro} : Baseline, BM3D, BF, CWT, CLEAN
\\
\cite{rethage2018wavenet} : WF
\\
\cite{zhang2016fast} : LRMC, DDTF
\\
\cite{li2019separating} : PF, CWT
\\
\cite{zhang2018ffdnet} : BM3D, WNNM, TNRD, DnCNN

\begin{table}[H]
    \renewcommand{\arraystretch}{1.3}
    \centering
    \caption{Baselines used in similar papers.}
    \label{tab:basedict}
    \begin{tabular}{p{0.2\linewidth}|p{0.5\linewidth}|p{0.15\linewidth}}
        \textbf{Acronym}&\textbf{Method}&\textbf{\# Uses}\\
        \toprule
        \bottomrule
        Baseline & no denoising & 1\\
        BF & Bilateral Filtering & 1\\
        WF & Wiener Filtering & 1\\
        CWT & Continuous Wavelet Transform & 2\\
        BM3D & Block-Matching and 3D filtering algorithm & 2 (3)\\
        BM4D & Black-Matching and 4D filtering algorithm & 1 (3)\\
        WNNM & Weighted Nuclear Norm Minimization & 1 (3)\\
        LRMC & Low Rank Matrix Completion & 1 (3)\\
        LRTA & Low Rank Tensor Approximation & 1 (3)\\
        LRTV & regularized Low-Rank matrix factorization Total Variation & 1 (3)\\
        LRMR & Low Rank Matrix Recovery & 1 (3)\\
        NMoG & Non-iid Mixture of Gaussians & 1\\
        DDTF & Data-Driven Tight Framework & 1\\
        \toprule
        \multicolumn{2}{c}{\textbf{Neural Networks}}\\
        \bottomrule
        DNN-SYMM & out=2048, depth=5, kernel=11 (citations=836) & 1\\
        DNN-CAUSAL & out=2048, depth=5, kernel=7 (citations=29) & 1\\
        RNN-NG & out=500, depth=5, context=3 (citations=373) & 1\\
        HSID-CNN & Residual CNN (citations=232) & 1\\
        TNRD & Trainable Nonlinear Reaction Diffusion (citations=966) & 1\\
        DnCNN & Denoising CNN (citations=4744) & 1\\
        \toprule
        \multicolumn{2}{c}{\textbf{Discarded}}\\
        \bottomrule
        MS & Microsoft Speech Enhancement & 1\\
        PF & Polynomial Fitting & 1\\
        CLEAN & 1\\
        \toprule
    \end{tabular}
\end{table}

\subsection{Evaluations}
\cite{ma2020enhanced} : PSNR, SSIM, SAM
\\
\cite{zhao2018convolutional} : SNR, LSD, MSE, WER, PESQ
\\
\cite{huang2018micro} : PSNR
\\
\cite{rethage2018wavenet} : SNR
\\
\cite{zhang2016fast} : PSNR
\\
\cite{li2019separating} : R
\\
\cite{zhang2018ffdnet} : PSNR

\begin{table}[H]
    \renewcommand{\arraystretch}{1.3}
    \centering
    \caption{Evaluations used in similar papers.}
    \label{tab:evaldict}
    \begin{tabular}{p{0.2\linewidth}|p{0.5\linewidth}|p{0.15\linewidth}}
        \textbf{Acronym}&\textbf{Method}&\textbf{\# Uses}\\
        \toprule
        \bottomrule
        SNR & Signal to Noise Ratio & 2 (6)\\
        PSNR & Peak Signal to Noise Ratio & 4 (6)\\
        SSIM & Structural SIMilarity & 1 (2)\\
        CW-SSIM & Complex Wavelet Structural SIMilarity & 1 (2)\\
        SAM & Spectral Angle Mapper & 1\\
        LSD & Log Spectral Distortion & 1\\
        MSE & Mean Squared Error & 1\\
        R & Correlation Coefficient & 1\\
        \toprule
        \multicolumn{2}{c}{\textbf{Discarded}}\\
        \bottomrule
        WER & Word Error Rate & 1\\
        PSEQ & Perceptual Evaluation of Speech Quality & 1\\
        \toprule
    \end{tabular}
\end{table}

==> sections/objects/fig_component_metrics.tex <==
\begin{figure}[!htb]
\centering

\centerline{\textbf{Number of stacked CDAEs versus denoising performance}}\medskip
\begin{minipage}[b]{\linewidth}
  \centering
  \centerline{\includegraphics[width=\textwidth]{figures/components_metrics.png}}
\end{minipage}
\caption{PSNR and SSIM scores from 1024 test samples after each CDAE component in DAARE.}
\label{fig:component_metrics}
\end{figure}

==> sections/objects/tab_cdae.tex <==
\begin{table}[!htb]
    \renewcommand{\arraystretch}{1.3}
    \centering
    \caption{The DAARE architecture. C$-$LN$-$LR($8,13\times5,1,(6,2)$) stands for a $13\times5$ Conv2d layer with $8$ output channels, a stride of $1$, a padding of $(6,2)$, followed by a LayerNorm and LeakyReLU with a negative slope of $0.2$.}
    \label{tab:cdae}
    \begin{tabular}{cx{0.33\linewidth}cx{0.33\linewidth}}
        \textbf{CDAE($\bullet$)}&\textbf{DAARE}\\
        \toprule
        \bottomrule
        $7\times$ C$-\bullet-$LR($8,13\times5,1,(6,2)$) & $3\times$ CDAE(LN)\\
        C($1,13\times5,1,(6,2)$) & $3\times$ CDAE\\
        Tanh &\\
        \toprule
    \end{tabular}
\end{table}

==> sections/objects/tab_ssr.tex <==
\begin{table}[!htb]
    \renewcommand{\arraystretch}{1.3}
    \centering
    \caption{The convolutional denoising autoencoder architecture. C($4,3\times3,2,1$)-LN-R stands for a $3\times3$ Conv2d layer with $4$ output channels, a stride of $1$, a padding of $1$, followed by LayerNorm and ReLU.}
    \label{tab:ssr}
    \begin{tabularx}{\linewidth}{>{\centering\arraybackslash}X}
        \textbf{Structural Super Resolution Block}\\
        \toprule
        \bottomrule
        C($4,3\times3,1,1$)-LN-R\\
        C($4,3\times3,1,1$)-LN-R\\
        C($4,3\times3,1,1$)\\
        Tanh\\
        \toprule
    \end{tabularx}
\end{table}
